Delaunay triangulation of manifolds

We present an algorithm for producing Delaunay triangulations of manifolds. The algorithm can accommodate abstract manifolds that are not presented as submanifolds of Euclidean space. Given a set of sample points and an atlas on a compact manifold, a manifold Delaunay complex is produced provided the transition functions are bi-Lipschitz with a constant close to 1, and the sample points meet a local density requirement; no smoothness assumptions are required. If the transition functions are smooth, the output is a triangulation of the manifold. The output complex is naturally endowed with a piecewise flat metric which, when the original manifold is Riemannian, is a close approximation of the original Riemannian metric. In this case the ouput complex is also a Delaunay triangulation of its vertices with respect to this piecewise flat metric.

==> Makefile <==
#
# Makefile for flat perturbation algorithm
# 20120921
#

TEXINPUTS := .:./styles//:

papers=manmesh inria_manmesh cgl_manmesh

default: manmesh.bbl

cgl: cgl_manmesh.bbl

inria: inria_manmesh.bbl

all: $(addsuffix .pdf,$(basename ${papers}))

bib: $(addsuffix .bbl,$(basename ${papers}))

%.pdf: %.tex *.tex
	pdflatex $<
	pdflatex $<

%.bbl: %.pdf *.bib
	bibtex $(basename $<)
	pdflatex $(basename $<)
	pdflatex $(basename $<)

clean:
	rm -f *.bbl *.blg *.aux *.out *.log *.brf *.thm *.toc \
$(addsuffix .pdf,$(basename ${papers}))

cleanmax: clean
	rm -f *~ lablst.pdf



==> quality_summary.tex <==
% -*- LaTeX -*-
% quality_summary.tex
% 20131010
%
% Observations about the  quality of the output mesh. Making a new file to replace the old quality.tex

\section{Output quality guarantees}
\label{sec:quality}

Given appropriate constraints on the input, \Thmref{thm:man.mesh}
guarantees that the output mesh, $\outmesh$, will be a manifold
simplicial complex. In this section, we justify the name
$\outmesh$ and examine the fitness of $\outmesh$ as a
representative of the input manifold $\man$.

\subsection{The output complex is a Delaunay complex}

Given $\pts \subset \man$, we define the set $\ppts \subset \man$ to be the perturbed point set produced by the algorithm, i.e., $\pts \to \ppts$ is given by $p \mapsto p' = \fcharti^{-1}(p'_i)$, where $i \in \apts$ is the label associated with $p \in \pts$.  If the metric on $\man$ is such that the coordinate maps $\fcharti$ themselves have low metric distortion, then the constructed complex $\outmesh$ is in fact the Delaunay complex of $\ppts \subset \man$.  This follows from the fact that in the local Euclidean coordinate frames we have ensured that the points have stable Delaunay triangulations.  Thus, using $\flakebnd = \frac{\pertbnd}{C}$ given by \Lemref{lem:loc.eucl.protect}, the stability result \Lemref{lem:del.metric.stability} leads, by the same reasoning that yields \Lemref{lem:stable.stars}, to the following:
\begin{thm}[Delaunay complex]
  \label{thm:output.del.cplx}
  Suppose that $\{(W_i,\fcharti)\}_{i \in \apts}$ is an atlas for the
  compact $m$-manifold $\man$, and the finite set $\pts \subset \man$
  is such that the conditions of \Secref{sec:input} are satisfied.
  Suppose also that $\man$ is equipped with a metric $\gdistM$, such that
  \begin{equation*}
    \abs{\disti{\fcharti(x)}{\fcharti(y)} - \distM{x}{y} } \leq \eta
    \disti{\fcharti(x)}{\fcharti(y)}, 
  \end{equation*}
  whenever $x$ and $y$ belong to
  $\fcharti^{-1}(\ballEm{p_i}{6\samconst_i})$.
  If
  \begin{equation*}
    \eta \leq \frac{\sparseconst^2}{2^{12}} \left( \frac{\pertbnd}{C} \right)^{2m+1},
  \end{equation*}
  and the conditions of \Thmref{thm:man.mesh} are met, then $\outmesh$
  is the Delaunay complex of $\ppts \subset \man$ with respect to
  $\gdistM$.
\end{thm}

Thus we construct a Delaunay complex for a metric that is locally well
approximated by the local Euclidean metrics. This is the standard
scenario: the manifold is sampled densely enough that natural local
coordinate charts have very low distortion and thus yield transition
functions which satisfy the requirements of \Thmref{thm:man.mesh}.


\subsection{A metric on the output complex}
\label{sec:out.metric}

The output mesh $\outmesh$ is an abstract simplicial complex, but it
admits a natural piecewise flat metric. This means that each simplex
in $\outmesh$ is identified with a geometric Euclidean simplex. This
is achieved by assigning lengths to the edges in $\outmesh$. If
$\asimplex{i,j}$ is an edge in $\outmesh$, then we give it the length
$\ell_{ij}$, where $\ell_{ij} = \frac{1}{2}(\disti{p'_i}{p'_j} +
\distj{p'_i}{p'_j})$.

We observe that with this assignment of edge lengths every simplex in
$\outmesh$ can be isometrically identified with the vertices of a
geometric Euclidean simplex. This is a consequence of our observations
in \Secref{sec:splx.distort}. Specifically, suppose $\splxs =
\asimplex{p_0, \ldots, p_k}$ is a simplex of points in $\rem$ and let
$\{\ell_{ij}\}_{0 \leq i \neq j \leq k}$ be a set of positive numbers
such that $\ell_{ij} = \ell_{ji}$ and $\abs{ \ell_{ij} - \norm{p_i -
    p_j} } \leq \metlipconst \longedge{\splxs}$.  Consider the $k
\times k$ symmetric matrix $G$ defined by $[G]_{ij} =
\frac{1}{2}(\ell_{0i}^2 + \ell_{0j}^2 - \ell_{ij}^2)$. Then using the
same notation and arguments as in \Lemref{lem:splx.gram}, we have that
$G = \transp{P}P + E$, and that $\sing{1}{E} \leq 4 k \metlipconst
\longedge{\splxs}^2$ if $\metlipconst \leq \frac{2}{3}$. It follows
then, using \Lemref{lem:bound.skP}, that $G$ is positive definite if
$\metlipconst < \left( \frac{\thickness{\splxs}}{2} \right)^2$, just
as was argued in \Lemref{lem:intrinsic.thick.distortion}. This means
that we may write $G = \transp{\tilde{P}}\tilde{P}$, where $\tilde{P}$
defines a non-degenerate Euclidean simplex whose edge lengths are
given by the numbers $\ell_{ij}$. The choice of $\tilde{P}$ is not
important: by considering the singular value decompositions it is
evident that if $\transp{Q}Q = \transp{\tilde{P}}\tilde{P}$, then
there is an orthogonal matrix $O$ such that $Q = O\tilde{P}$.

For any $\tsplxs \in \outmesh$ we may compare its edge lengths to those of the corresponding simplex $\splxs \in \str{p'_i;\delof{\ppts_i}}$, where $i$ is the label of one of the vertices of $\tsplxs$. Under the assumptions of \Lemref{lem:loc.eucl.protect}, the condition $\metlipconst < \left( \frac{\thickness{\splxs}}{2} \right)^2$ is satisfied, and the above argument shows that $\tsplxs$ may be identified with a Euclidean simplex.


\subsection{Homeomorphism guarantee in the smooth case}
\label{sec:homeomorphims}

If the coordinate charts have small metric distortion, then the sampling radii in the coordinate patches imply that $\ppts$ satisfies some constant sampling radius, $\samconst$, with respect to the metric on the compact manifold. For a Riemannian manifold, a natural choice for a coordinate chart is the inverse of the exponential map, e.g., $\fcharti = \exp_{p_i}^{-1}|_{W_i}$. Then the metric distortion of the coordinate chart $\fcharti$ decreases as the diameter of the domain $W_i$ decreases; this is a consequence of a theorem due to Rauch~\cite[Thm IX.2.3, p. 390]{chavel2006}.  This means that for $\samconst$ sufficiently small, $\outmesh$ will be homeomorphic to $\man$. This can be argued by appealing to the homeomorphism demonstration detailed by Boissonnat and Ghosh~\cite{boissonnat2014tancplx.dcg}, for example.

We employ the Nash embedding theorem, which ensures that $\man$ may be isometrically embedded in some ambient Euclidean space $\amb$. 
When the neighbourhoods $W_i$ are small, the restricted ambient metric $\gdistRM$ is a close approximation to the intrinsic metric $\gdistM$ on the manifold. (See \cite[Lemma 3.7]{boissonnat2013stab2.inria}, for example.) In other words the identity map $(W_i, \gdistRM) \to (W_i, \gdistM)$ is an $\eta$-distortion map, where the magnitude of $\eta$ decreases with the diameter of $W_i$.

This means that when $\samconst$ is small enough, the stability theorem \cite[Theorem 4.17]{boissonnat2013stab1} ensures that not only is $\outmesh$ the Delaunay complex of $\ppts \subset \man$ with respect to the intrinsic metric $\gdistM$, but also with respect to the restricted ambient metric $\gdistRM$. We are also assured, by \Lemref{lem:intrinsic.thick.distortion}, that the simplices of $\outmesh$ satisfy some lower bound $\tilde{\Upsilon}_0$ on their thickness when they are realised as Euclidean simplices in the ambient space, i.e., when the edge lengths between vertices are given by the Euclidean distance in $\amb$. These observations place $\outmesh$ in the setting considered by Boissonnat and Ghosh~\cite{boissonnat2014tancplx.dcg} in the context of the tangential Delaunay complex, and the same argument demonstrates that $\outmesh$ is homeomorphic to $\man$. The homeomorphism construction of Boissonnat and Ghosh requires the submanifold $\man$ to be smooth.


\subsection{Discussion}
\label{sec:discussion}

We are able to quantify the conditions under which $\outmesh$ will be a manifold Delaunay complex. These are already stringent conditions on the metric, although smoothness is not required. However, we make no claim that $\outmesh$ is homeomorphic to $\man$, except for certain smooth transition functions, and for ``sufficiently dense'' sampling. The specification of concrete sampling criteria that are sufficient to guarantee a homeomorphic complex is still an open problem. A careful construction of a homeomorphism will also enable us to quantify its metric distortion, i.e., to quantify a bound on the Gromov-Hausdorff distance between $\man$ and $\outmesh$, when the latter is equipped with the metric described in \Secref{sec:out.metric}, for example.

When the differences in the metrics are sufficiently small, the Delaunay stability results imply that not only is $\outmesh$ a Delaunay complex for $\ppts \subset \man$, but it is also the Delaunay complex of its vertices associated with its own intrinsic metric. Such meshes are of interest in discrete differential geometry \cite{glickenstein2005, dyer2010thesis, hirani2012}.



==> review.tex <==
% -*- LaTeX -*-
% review.tex
% 20130609
% Review of the flat perturbation algorithm

\section{Review of the algorithm for flat manifolds}
\label{sec:review}

We review the perturbation algorithm
\cite{boissonnat2014flatpert} for points in Euclidean space. The
algorithm for more general manifolds is a natural extension of this.

We consider a finite set $\pts \subset \rem$.  A simplex $\splxs
\subset \pts$ is a finite collection of points: $\splxs =
\asimplex{p_0, \ldots, p_k}$. We work with abstract simplices, and in
particular $x \in \splxs$ means $x$ is a vertex of $\splxs$.  The
dimension of a simplex is one less than the number of vertices, and a
$j$-dimensional simplex is a $j$-simplex. The dimension, if it is
important, may be indicated with a superscript, as in $\splxs^m$.  The
notation $\splxs \leq \splxt$ indicates that $\splxs$ is a face of
$\splxt$ (i.e., a subset), and $\splxs < \splxt$ means that it is a
proper face. The join of two simplices, $\splxjoin{\splxt}{\splxs}$,
is the union of their vertices.  By the standard abuse of notation, a
point $p$ may represent the $0$-simplex $\{p\}$.

If $\splxs \subset \rem$, then we freely talk about standard geometric
properties, such as the diameter, $\longedge{\splxs}$, and the length
of the shortest edge $\shortedge{\splxs}$. For $p \in \splxs$,
$\opface{p}{\splxs}$ is the facet opposite $p$, and
$\splxalt{p}{\splxs}$ is the \defn{altitude} of $p$ in $\splxs$, i.e.,
$\splxalt{p}{\splxs}= \distEm{p}{\affhull{\opface{p}{\splxs}}}$.

The \defn{thickness} of $\splxs^j$ is defined as
\begin{equation*}
  \thickness{\splxs^j} =
  \begin{cases}
    1& \text{if $j=0$} \\
    \min_{p \in \splxs^j} \frac{\splxalt{p}{\splxs^j}}{j
      \longedge{\splxs^j}}& \text{otherwise.}
  \end{cases}
\end{equation*}
It is a measure of the quality of the simplex. If $\thickness{\splxs}
= 0$, then $\splxs$ is \defn{degenerate}.  We say that $\splxs$ is
$\thickbnd$-thick, if $\thickness{\splxs} \geq \thickbnd$. If $\splxs$
is $\thickbnd$-thick, then so are all of its faces.

A \defn{circumscribing ball} for a simplex $\splxs$ is any $m$-dimensional ball that contains the vertices of $\splxs$ on its boundary.  A degenerate simplex may not admit any circumscribing ball.  If $\splxs$ admits a circumscribing ball, then it has a \defn{circumcentre}, $\circcentre{\splxs}$, which is the centre of the unique smallest circumscribing ball for $\splxs$. The radius of this ball is the \defn{circumradius} of $\splxs$, denoted $\circrad{\splxs}$. A degenerate simplex $\splxs$ may or may not have a circumcentre and circumradius; we write $\circrad{\splxs} < \infty$ to indicate that it does.  In this case we can also define the \defn{diametric sphere} as the boundary of the smallest circumscribing ball: $\diasphere{\splxs} = \bdry{\ballEm{\circcentre{\splxs}}{\circrad{\splxs}}}$, and the \defn{circumsphere}: $\circsphere{\splxs} = \diasphere{\splxs} \cap \affhull{\splxs}$. If $\splxs \leq \splxt$, then $\circsphere{\splxs} \subseteq \circsphere{\splxt}$, and if $\dim \splxs = m$, then $\circsphere{\splxs} = \diasphere{\splxs}$.

A ball $\ballEm{c}{r}$ is open, and $\cballEm{c}{r}$ is its closure.
The Delaunay complex, $\delP$ is the (abstract) simplicial complex
defined by the criterion that a simplex belongs to $\delP$ if it has a
circumscribing ball whose intersection with $\pts$ is empty. An
$m$-simplex $\splxs^m$ is \defn{$\delta$-protected} if
$\cballEm{\circcentre{\splxs^m}}{\circrad{\splxs^m} + \delta} \cap
\pts = \splxs^m$.

A point set whose Delaunay $m$-simplices are $\delta$-protected has
quantifiable stability properties with respect to perturbations of the
points, or of the metric \cite{boissonnat2013stab1}. In order for
comparisons between radii, edge lengths, and $\delta$, to be
meaningful, we introduce a common ``unit''. Let $\samconst$ be an
upper bound on the circumradii of the Delaunay balls centred in
$\convhull{\pts}$, and let $\sparseconst \samconst$ be the minimum
distance between distinct points in $\pts$. Since $\pts$ is finite,
$\samconst$ and $\sparseconst$ exist, with the only additional required
assumptions on $\pts$ being that $\affhull{\pts} = \rem$, and that the
points in $\pts$ are distinct.

If $D \subset \rem$, then $\pts$ is \defn{$\samconst$-dense} for $D$
if $\distEm{x}{\pts} < \samconst$ for all $x \in D$. If no domain is
specified, $\pts$ is $\samconst$-dense if it is $\samconst$-dense for
\begin{equation*}
%  \label{eq:contracted.hull}
  D_\samconst(\pts) = \{ x \in \convhull{\pts} \, | \,
  \distEm{x}{\bdry{\convhull{\pts}}} \geq \samconst \}.
\end{equation*}
We refer to $\samconst$ as the \defn{sampling radius}.  The set $\pts$
is \defn{$\sparseconst \samconst$-separated} if $\distEm{p}{q} \geq
\sparseconst \samconst$ for all $p,q \in \pts$, and $\pts$ is a
\ueset\ (for $D$) if it is $\sparseconst \samconst$-separated, and
$\samconst$-dense (for $D$).

The Delaunay stability results require an upper bound on the
circumradii of the Delaunay balls. The \defn{Delaunay complex of
  $\pts$ restricted to $D$} is the subcomplex consisting of simplices
that have a Delaunay ball centred in $D$. We denote the Delaunay
complex of $\pts$ restricted to $D_{\samconst}(P)$ by $\rdelpts$, and
observe that the Delaunay balls for simplices in $\rdelpts$ have radii
smaller than $\samconst$, and in particular, $\circrad{\splxs} <
\samconst$ if $\splxs \in \rdelpts$.

The goal is to produce a perturbed point set $\ppts$ such that the
Delaunay $m$-simplices of $\rdelppts$ are \defn{$\delta$-protected}.
A \defn{$\pertconst$-perturbation} of a \ueset\ $\pts \subset \rem$ is
a bijective application $\pert: \pts \to \ppts \subset \rem$ such that
$\distEm{\pert(p)}{p} \leq \pertconst$ for all $p \in \pts$.
Unless otherwise specified, a \defn{perturbation} will always refer to
a $\pertconst$-perturbation, with $\pertconst = \pertbnd \samconst$
for some
\begin{equation}
  \label{eq:pertbnd}
  \pertbnd \leq \frac{\sparseconst}{4}.
\end{equation}
We also refer to $\ppts$ itself as a perturbation of $\pts$.  We
generally use $p'$ to denote the point $\pert(p) \in \ppts$, and
similarly, for any point $q' \in \ppts$ we understand $q$ to be its
preimage in $\pts$.

The ``perturbations'' constrained by \Eqnref{eq:pertbnd}
are not particularly ``small'', and in particular, we do not expect a
close relationship between $\delP$ and $\delof{\ppts}$. However, we do
have the useful observation \cite[Lemma
2.2]{boissonnat2014flatpert} that $\ppts$ is a \pueset:
\begin{lem}
  \label{lem:perturb.Delone}
  If $\pts \subset \rem$ is a \ueset, and $\ppts$ is a perturbation of
  $\pts$, then $\ppts$ is a \pueset, where
  \begin{itemize}
  \item $\psamconst = (1 + \pertbnd)\samconst \leq \frac{5}{4}\samconst$,
    and
  \item $\psparseconst = \frac{\sparseconst - 2\pertbnd}{1 + \pertbnd}
    \geq \frac{2}{5} \sparseconst$.
  \end{itemize}
\end{lem}

The construction of the algorithm is based on the concept of \defn{forbidden configurations}, which are specific simplices that indicate the presence Delaunay $m$-simplices that are not sufficiently thick, or not $\delta$-protected. Forbidden configurations possess the \defn{$\hoopbnd$-hoop property}. A simplex has the $\hoopbnd$-hoop property if every vertex lies close to the circumsphere of the opposing facet. Specifically, for $\hoopbnd > 0$, a simplex $\splxt$ has the $\hoopbnd$-hoop property if, for every $p \in \splxt$,
\begin{equation*}
  \distEm{p}{\circsphere{\opface{p}{\splxt}}} \leq \hoopbnd
  \circrad{\opface{p}{\splxt}} < \infty.
\end{equation*}

We will first sketch the argument that shows that Delaunay $m$-simplices that are not $\delta$-protected indicate the presence of forbidden configurations.  Then we will describe how the hoop property is exploited in the perturbation algorithm.

A forbidden configuration is a specific kind of poorly shaped simplex that has the property that \emph{all} its altitudes are small. A simplex that has an upper bound on its thickness will also have an altitude that is subjected to an upper bound, but in order to obtain a useful upper bound on all of the altitudes, we need a more refined measure of simplex quality. Given a positive parameter $\flakebnd \leq 1$, we say that $\splxs$ is \defn{$\flakebnd$-good} if for all $\splxs^j \leq \splxs$, we have $\thickness{\splxs^j} \geq \flakebnd^j$, where $\flakebnd^j$ is the $j^{\text{th}}$ power of $\flakebnd$.  A simplex that is $\flakebnd$-good is necessarily $\flakebnd^m$-thick, but the converse is not generally true. A \defn{$\flakebnd$-flake} is a simplex that is not $\flakebnd$-good, but whose facets all are.  The altitudes of a flake are subjected to an upper bound proportional to $\flakebnd$.

If a simplex is not $\flakebnd$-good, then it necessarily contains a
face that is a flake. This follows easily from the observation that
$\thickness{\splxs} = 1$ if $\splxs$ is a $1$-simplex. If $\splxs^m
\in \delP$ is not $\delta$-protected, then there is a $q \in \pts
\setminus \splxs^m$ that is within a distance $\delta$ of the
circumsphere of $\splxs^m$. Since $\splxjoin{q}{\splxs^m}$ is
$(m+1)$-dimensional, it is degenerate, and therefore has a face
$\splxt$ that is a $\flakebnd$-flake. Such a $\splxt$ is a forbidden
configuration. 

The bound on the altitudes, together with the stability property of
circumscribing balls of thick simplices, allows us to demonstrate that
forbidden configurations have the hoop property. In addition to the
two parameters that describe a \ueset, forbidden configurations depend
on the flake parameter $\flakebnd$, as well as the parameter
$\delta_0$, which governs the protection via the requirement $\delta =
\delta_0 \sparseconst \samconst$. We do not need to explicitly define
forbidden configurations here. Instead, we make reference to the
following summary \cite[Theorem 3.10]{boissonnat2014flatpert} of
properties of forbidden configurations in $\ppts$:
\begin{lem}[Properties of forbidden configurations]
%  \label{thm:no.hoops.implies.protection}
  \label{lem:prop.forbid.cfg} % for the properties
  Suppose that $\pts \subset \rem$ is a \ueset\ and that $\ppts$ is a
  perturbation of $\pts$.
%  such that there is no simplex $\splxt \subset \ppts$ that
  If
  \begin{equation}
    \label{eq:dnobnd}
    \delta_0 \leq \flakebnd^{m+1} \quad \text{and} \quad \flakebnd
    \leq \frac{2\sparseconst^2 }{75},
  \end{equation}
  then every forbidden configuration $\splxt \subset \ppts$ 
  satisfies \emph{all} of the following properties:
  \begin{enumerate}[label={$\mathcal{P}$\arabic*}]
  \item \label{hyp:clean.hoop.bnd}
    Simplex $\splxt$ has the \hoop\ property, with
%    $\hoopbnd = 2 \left( \frac{16}{\sparseconst} \right)^3
%    \flakebnd$.
    $\hoopbnd = \frac{ 2^{13} \flakebnd }{\sparseconst^3}$.
  \item \label{hyp:clean.facet.rad.bnd}
    For all $p \in \splxt$,
    $\circrad{\splxtp} < 2\samconst$.
  \item \label{hyp:diam.bnd} 
   $\longedge{\splxt} < \frac{5}{2}(1 +
   \frac{1}{2}\delta_0\sparseconst)\samconst$. 
  \item \label{hyp:good.facets}
    Every facet of $\splxt$ is $\flakebnd$-good.
  \end{enumerate}
  % If
  % \begin{equation}
  %   \label{eq:dnobnd}
  %   \delta_0 \leq \flakebnd^{m+1} \quad \text{and} \quad \flakebnd
  %   \leq \frac{2\sparseconst^2 }{75},
  % \end{equation}
%  then $\ppts$ contains no \dgconfig s.
 % and thus all the $m$-simplices
 %  in $\rdelppts$ are $\flakebnd$-good and $\delta$-protected, with
 %  $\delta = \delta_0 \psparseconst \psamconst$.
\end{lem}

The algorithm focuses on Property~\ref{hyp:clean.hoop.bnd} of
forbidden configurations.  A critical aspect of this property is its
symmetric nature; if we can ensure that $\splxt$ has one vertex that is
not too close to its opposite facet, then $\splxt$ cannot be a
forbidden configuration. 

Using Property~\ref{hyp:diam.bnd}, we can find, for each $p \in
\pts$, a complex $\mathcal{S}_p$ consisting all simplices $\splxs \in
\pts$ such that after perturbations $\splxjoin{p}{\splxs}$ could be a
forbidden configuration. 


The algorithm proceeds by perturbing each point $p \in \pts$ in turn,
such that each point is only visited once. The perturbation $p \mapsto
p'$ is found by randomly trying perturbations $p \mapsto x$ until it
is found that $x$ is a \defn{good perturbation}. A good perturbation
is one in which $\distEm{x}{\circsphere{\splxs}} > 2\hoopbnd
\samconst$ for all $\splxs \in \mathcal{S}_p(\ppts)$, where
$\mathcal{S}_p(\ppts)$ is the complex in the current perturbed point
set whose simplices correspond to those in $\mathcal{S}_p$.

A volumetric argument based on the finite number of simplices in
$\mathcal{S}_p$, the small size of $\hoopbnd$, and the volume of the
ball $\ballEm{p}{\pertbnd \samconst}$ of possible perturbations of
$p$, reveals a high probability that $p \mapsto x$ will be a good
perturbation, and thus ensures that the algorithm will terminate.

Upon termination there will be no forbidden configurations in $\ppts$,
because every perturbation $p \mapsto p'$ ensures that there are no
forbidden configurations incident to $p'$ in the current point set,
and no new forbidden configurations are introduced. 

